Rethinking Conversational Recommendations: Is Decision Tree All You Need?

Conversational recommender systems (CRS) dynamically obtain the user preferences via multi-turn questions and answers. The existing CRS solutions are widely dominated by deep reinforcement learning algorithms. However, deep reinforcement learning methods are often criticised for lacking interpretability and requiring a large amount of training data to perform. In this paper, we explore a simpler alternative and propose a decision tree based solution to CRS. The underlying challenge in CRS is that the same item can be described differently by different users. We show that decision trees are sufficient to characterize the interactions between users and items, and solve the key challenges in multi-turn CRS: namely which questions to ask, how to rank the candidate items, when to recommend, and how to handle negative feedback on the recommendations. Firstly, the training of decision trees enables us to find questions which effectively narrow down the search space. Secondly, by learning embeddings for each item and tree nodes, the candidate items can be ranked based on their similarity to the conversation context encoded by the tree nodes. Thirdly, the diversity of items associated with each tree node allows us to develop an early stopping strategy to decide when to make recommendations. Fourthly, when the user rejects a recommendation, we adaptively choose the next decision tree to improve subsequent questions and recommendations. Extensive experiments on three publicly available benchmark CRS datasets show that our approach provides significant improvement to the state of the art CRS methods.

==> oldbib.tex <==
% @article{young2013pomdp,
%   title={Pomdp-based statistical spoken dialog systems: A review},
%   author={Young, Steve and Ga{\v{s}}i{\'c}, Milica and Thomson, Blaise and Williams, Jason D},
%   journal={Proceedings of the IEEE},
%   volume={101},
%   number={5},
%   pages={1160--1179},
%   year={2013},
%   publisher={IEEE}
% }


% @inproceedings{yee2003faceted,
%   title={Faceted metadata for image search and browsing},
%   author={Yee, Ka-Ping and Swearingen, Kirsten and Li, Kevin and Hearst, Marti},
%   booktitle={Proceedings of the SIGCHI conference on Human factors in computing systems},
%   pages={401--408},
%   year={2003}
% }


% @inproceedings{kato2016suggest,
%   title={To suggest, or not to suggest for queries with diverse intents: Optimizing search result presentation},
%   author={Kato, Makoto P and Tanaka, Katsumi},
%   booktitle={Proceedings of the Ninth ACM International Conference on Web Search and Data Mining},
%   pages={133--142},
%   year={2016}
% }

% @inproceedings{mccarthy2010experience,
%   title={Experience-based critiquing: Reusing critiquing experiences to improve conversational recommendation},
%   author={McCarthy, Kevin and Salem, Yasser and Smyth, Barry},
%   booktitle={International Conference on Case-Based Reasoning},
%   pages={480--494},
%   year={2010},
%   organization={Springer}
% }

% @book{salton1971smart,
%   title={The SMART retrieval system—experiments in automatic document processing},
%   author={Salton, Gerard},
%   year={1971},
%   publisher={Prentice-Hall, Inc.}
% }

% @article{sukhbaatar2015end,
%   title={End-to-end memory networks},
%   author={Sukhbaatar, Sainbayar and Szlam, Arthur and Weston, Jason and Fergus, Rob},
%   journal={arXiv preprint arXiv:1503.08895},
%   year={2015}
% }


% @incollection{chu1998evidential,
%   title={An evidential model for tracking initiative in collaborative dialogue interactions},
%   author={Chu-Carroll, Jennifer and Brown, Michael K},
%   booktitle={Computational Models of Mixed-Initiative Interaction},
%   pages={49--87},
%   year={1998},
%   publisher={Springer}
% }


% @inproceedings{radlinski2017theoretical,
%   title={A theoretical framework for conversational search},
%   author={Radlinski, Filip and Craswell, Nick},
%   booktitle={Proceedings of the 2017 conference on conference human information interaction and retrieval},
%   pages={117--126},
%   year={2017}
% }

% @inproceedings{zhang2018towards,
%   title={Towards conversational search and recommendation: System ask, user respond},
%   author={Zhang, Yongfeng and Chen, Xu and Ai, Qingyao and Yang, Liu and Croft, W Bruce},
%   booktitle={Proceedings of the 27th acm international conference on information and knowledge management},
%   pages={177--186},
%   year={2018}
% }

% @misc{argerich2020,
% title = {When to use Reinforcement Learning (and when not to)},
% author = {Mauricio Fadel Argerich},
% url = {https://medium.com/swlh/when-to-use-reinforcement-learning-and-when-not-to-919557dd34a},
% year = {2020}
% }


% @inproceedings{lei2020estimation,
%   title={Estimation-action-reflection: Towards deep interaction between conversational and recommender systems},
%   author={Lei, Wenqiang and He, Xiangnan and Miao, Yisong and Wu, Qingyun and Hong, Richang and Kan, Min-Yen and Chua, Tat-Seng},
%   booktitle={Proceedings of the 13th International Conference on Web Search and Data Mining},
%   pages={304--312},
%   year={2020}
% }


% @article{deng2021unified,
%   title={Unified Conversational Recommendation Policy Learning via Graph-based Reinforcement Learning},
%   author={Deng, Yang and Li, Yaliang and Sun, Fei and Ding, Bolin and Lam, Wai},
%   journal={arXiv preprint arXiv:2105.09710},
%   year={2021}
% }


% @article{kang2019recommendation,
%   title={Recommendation as a communication game: Self-supervised bot-play for goal-oriented dialogue},
%   author={Kang, Dongyeop and Balakrishnan, Anusha and Shah, Pararth and Crook, Paul and Boureau, Y-Lan and Weston, Jason},
%   journal={arXiv preprint arXiv:1909.03922},
%   year={2019}
% }

% @inproceedings{tao2019fact,
%   title={The fact: Taming latent factor models for explainability with factorization trees},
%   author={Tao, Yiyi and Jia, Yiling and Wang, Nan and Wang, Hongning},
%   booktitle={Proceedings of the 42nd International ACM SIGIR Conference on Research and Development in Information Retrieval},
%   pages={295--304},
%   year={2019}
% }

